Analyzing the Effectiveness of Listwise Reranking with Positional Invariance on Temporal Generalizability

This working note outlines our participation in the retrieval task at CLEF 2024. We highlight the considerable gap between studying retrieval performance on static knowledge documents and understanding performance in real-world environments. Therefore, Addressing these discrepancies and measuring the temporal persistence of IR systems is crucial. By investigating the LongEval benchmark, specifically designed for such dynamic environments, our findings demonstrate the effectiveness of a listwise reranking approach, which proficiently handles inaccuracies induced by temporal distribution shifts. Among listwise rerankers, our findings show that ListT5, which effectively mitigates the positional bias problem by adopting the Fusion-in-Decoder architecture, is especially effective, and more so, as temporal drift increases, on the test-long subset.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> prompt_boxes/prompt_publish_date_extraction.tex <==
\begin{tcolorbox}[title=Published Date Extraction Prompt]
\textbf{System}: \\
You are TimeIndexer, an intelligent assistant that helps improve the search quality by correctly predicting and indexing the time information of documents. \\
Your answer must strictly adhere to the output format. Do not say any word or explain. \\

\textbf{Input}: \\
You will be given a document, and your job is to predict the publication date of the document in the format of "Month Year", which is "\%B-\%Y" in strftime format. \\
Which will then be added to the document to enhance the search quality of documents in the aspect of time.\\ \\ 
Document: \{\{Document\}\} \\
Predict the publication date of the given document. The output format should be a single "Month Year", or "\%B-\%Y" in strftime format, such as May 2023, April 1998, December 2021, or February 2019. \\
Only response a single publication date, do not say any word or explain.
\end{tcolorbox}

==> sections/A_Acknowledgements.tex <==
\begin{acknowledgments}
  Thanks to the developers of ACM consolidated LaTeX styles
  \url{https://github.com/borisveytsman/acmart} and to the developers
  of Elsevier updated \LaTeX{} templates
  \url{https://www.ctan.org/tex-archive/macros/latex/contrib/els-cas-templates}.  
\end{acknowledgments}

==> tables/extra_results_test_long.tex <==
\begin{table*}[t]
\centering
\caption{
Comparative evaluation between baselines and ours on LongEval 2024 competition test-long datasets. The best performance on each dataset for each method is highlighted in bold and the second base is underlined. (|C| indicates whole corpus.)}
\label{tab:extra-result-test-long}
\scalebox{0.85}{
\def\arraystretch{1.1}
\begin{tabular}{lc|lc|ccccc}
\hline
\multicolumn{2}{c|}{Source} &
  \multicolumn{1}{c}{Retrieval Model} &
  \multicolumn{1}{c|}{Param} &
  \multicolumn{5}{c}{Test-Long} \\
\multicolumn{1}{c}{Prev.} &
  \multicolumn{1}{c|}{Top-k (return-k)} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c}{nDCG@10} &
  \multicolumn{1}{c}{nDCG@100} &
  \multicolumn{1}{c}{MAP@100} &
  \multicolumn{1}{c}{P@10} &
  \multicolumn{1}{c}{Recall@100} \\ \hline
None &
  |C| &
  BM25 &
  - &
  13.74\% &
  18.57\% &
  9.70\% &
  10.30\% &
  29.45\% \\
None &
  |C| &
  RepLLaMA &
  7B &
  17.17\% &
  22.29\% &
  12.35\% &
  12.82\% &
  {\ul 33.81\%} \\ \hline
BM25 &
  100 &
  MonoT5 &
  3B &
  17.67\% &
  21.27\% &
  12.74\% &
  13.13\% &
  29.45\% \\
BM25 &
  100 &
  ListT5 &
  3B &
  18.21\% &
  21.65\% &
  13.23\% &
  13.40\% &
  29.45\% \\
BM25 &
  100 &
  RankZephyr &
  7B &
  17.70\% &
  21.47\% &
  12.79\% &
  12.57\% &
  29.45\% \\
BM25 &
  100 &
  RankVicuna &
  7B &
  15.28\% &
  19.91\% &
  11.12\% &
  10.92\% &
  29.45\% \\
BM25 &
  100 &
  Llama3 &
  8B &
  12.72\% &
  17.65\% &
  8.76\% &
  10.15\% &
  29.45\% \\ \hline
RepLLaMA &
  100 &
  MonoT5 &
  3B &
  18.77\% &
  23.27\% &
  13.54\% &
  14.15\% &
  {\ul 33.81\%} \\
RepLLaMA &
  100 &
  ListT5 &
  3B &
  \textbf{19.45\%} &
  \textbf{23.80\%} &
  \textbf{14.24\%} &
  \textbf{14.38\%} &
  {\ul 33.81\%} \\
RepLLaMA &
  100 &
  RankZephyr &
  7B &
  19.18\% &
  23.75\% &
  14.04\% &
  13.96\% &
  {\ul 33.81\%} \\
RepLLaMA &
  100 &
  RankVicuna &
  7B &
  16.46\% &
  22.19\% &
  12.17\% &
  11.87\% &
  {\ul 33.81\%} \\
RepLLaMA &
  100 &
  Llama3 &
  8B &
  16.22\% &
  21.41\% &
  11.40\% &
  12.65\% &
  {\ul 33.81\%} \\
\hline
\hline
(Ours) &
  &
  &
  &
 \multirow{4}{*}{\ul 19.33\%} &
 \multirow{4}{*}{{\ul 23.76\%}} &
 \multirow{4}{*}{{\ul 14.15\%}} &
 \multirow{4}{*}{\ul{14.29\%}} &
 \multirow{4}{*}{\textbf{34.04}\%} \\ 
BM25 &
  1000 (100) &
  RepLLaMA &
  7B &
  &
  &
  &
  &
  \\ 
\quad $\rightarrow$ RepLLaMA &
  100 (70) &
  ListT5 &
  3B &
  &
  &
  &
  &
  \\ 
+ RepLLaMA &
  (930) &
  - &
  - &
  &
  &
  &
  &
  \\ 
\hline
\end{tabular}
}
\end{table*}

==> tables/extra_results_test_short.tex <==
\begin{table*}[t]
\centering
\caption{
Comparative evaluation between baselines and ours on LongEval 2024 competition test-short datasets. The best performance on each dataset for each method is highlighted in bold and the second base is underlined. (|C| indicates whole corpus.)}
\label{tab:extra-result-test-short}
\scalebox{0.85}{
\def\arraystretch{1.1}
\begin{tabular}{lc|lc|ccccc}
\hline
\multicolumn{2}{c|}{Source} &
  \multicolumn{1}{c}{Model} &
  \multicolumn{1}{c|}{Param} &
  \multicolumn{5}{c}{Test-Short} \\
\multicolumn{1}{c}{Prev.} &
  \multicolumn{1}{c|}{Top-k (return-k)} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c}{nDCG@10} &
  \multicolumn{1}{c}{nDCG@100} &
  \multicolumn{1}{c}{MAP@100} &
  \multicolumn{1}{c}{P@10} &
  \multicolumn{1}{c}{Recall@100} \\ \hline
None &
  |C| &
  BM25 &
  - &
  16.09\% &
  24.40\% &
  13.44\% &
  12.82\% &
  42.45\% \\
None &
  |C| &
  RepLLaMA &
  7B &
  21.04\% &
  29.82\% &
  17.63\% &
  16.88\% &
  {\ul 49.28\%} \\ \hline
BM25 &
  100 &
  MonoT5 &
  3B &
  21.49\% &
  28.16\% &
  17.67\% &
  16.78\% &
  42.45\% \\
BM25 &
  100 &
  ListT5 &
  3B &
  22.41\% &
  28.62\% &
  18.32\% &
  17.56\% &
  42.45\% \\
BM25 &
  100 &
  RankZephyr &
  7B &
  22.72\% &
  29.06\% &
  18.74\% &
  17.23\% &
  42.45\% \\
BM25 &
  100 &
  RankVicuna &
  7B &
  18.68\% &
  26.41\% &
  16.14\% &
  14.79\% &
  42.45\% \\
BM25 &
  100 &
  Llama3 &
  8B &
  15.03\% &
  23.49\% &
  12.35\% &
  12.57\% &
  42.45\% \\ \hline
RepLLaMA &
  100 &
  MonoT5 &
  3B &
  21.72\% &
  30.35\% &
  18.46\% &
  17.35\% &
  {\ul 49.28\%} \\ 
RepLLaMA &
  100 &
  ListT5 &
  3B &
  {\ul 23.11\%} &
  31.27\% &
  {\ul 19.51\%} &
  {\ul 18.17\%} &
  {\ul 49.28\%} \\
RepLLaMA &
  100 &
  RankZephyr &
  7B &
  \textbf{23.96\%} &
  \textbf{31.90\%} &
  \textbf{20.04\%} &
  \textbf{18.94\%} &
  {\ul 49.28\%} \\ 
RepLLaMA &
  100 &
  RankVicuna &
  7B &
  19.74\% &
  29.22\% &
  17.32\% &
  15.99\% &
  {\ul 49.28\%} \\ 
RepLLaMA &
  100 &
  Llama3 &
  8B &
  20.19\% &
  29.08\% &
  16.45\% &
  16.68\% &
  {\ul 49.28\%} \\ 
\hline
\hline
(Ours) &
  &
  &
  &
 \multirow{4}{*}{23.00\%} &
 \multirow{4}{*}{{\ul 31.36\%}} &
 \multirow{4}{*}{19.50\%} &
 \multirow{4}{*}{18.09\%} &
 \multirow{4}{*}{\textbf{49.90\%}} \\ 
BM25 &
  1000 (100) &
  RepLLaMA &
  7B &
  &
  &
  &
  &
  \\ 
\quad $\rightarrow$ RepLLaMA &
  100 (70) &
  ListT5 &
  3B &
  &
  &
  &
  &
  \\ 
+ RepLLaMA &
  (930) &
  - &
  - &
  &
  &
  &
  &
  \\ 
\hline
\end{tabular}
}
\end{table*}

==> tables/main_mid_submission.tex <==
\begin{table*}[t]
\centering
\caption{Comparative evaluation of \textbf{nDCG@10} and \textbf{nDCG@100} scores between baselines and ours on 2023 competition dataset. The best performance on each dataset and each metric for each method is highlighted in bold.}
\label{tab:ndcg10}
\scalebox{0.9}{
\def\arraystretch{1.2}
\begin{tabular}{c|c|ccc|c}
\noalign{\hrule height 1pt}
\multicolumn{1}{c|}{\textbf{Metric}} & \textbf{Method}  & \textbf{Train} & \textbf{Test-Long} & \textbf{Test-Short} & \textbf{Average} \\ 
\hline
\multirow{6}{*}{nDCG@10} &
\multicolumn{1}{l|}{BM25 (uncleaned)}      & 16.88 & 17.37 & 17.47 & 17.24 \\
& \multicolumn{1}{l|}{BM25}                 & 16.76 & 17.38 & 17.66 & 17.27 \\
                      & \multicolumn{1}{l|}{BM25 + MonoT5}        & 22.78 & 23.54 & 23.09 & 23.14 \\
                      & \multicolumn{1}{l|}{BM25 + MonoT5 + 
                      date Document}        & - & 23.21 & 22.81 & - \\
                      & \multicolumn{1}{l|}{BM25 + MonoT5 + date Query}        & - & 19.13 & 19.4 & - \\
                      & \multicolumn{1}{l|}{BM25 + ListT5 + ours} & \textbf{24.22} & \textbf{25.21} & \textbf{24.26} & \textbf{24.56} \\
\noalign{\hrule height 1pt}
\multirow{6}{*}{nDCG@100} &
\multicolumn{1}{l|}{BM25 (uncleaned)}      & 24.23 & 25.27 & 24.72 & 24.74 \\
& \multicolumn{1}{l|}{BM25}                 & 24.20 & 25.46 & 25.02 & 24.89 \\
                      & \multicolumn{1}{l|}{BM25 + MonoT5}        & 28.21 & 29.6 & 28.7 & 28.84 \\
                      & \multicolumn{1}{l|}{BM25 + MonoT5 + 
                      date Document}        & - & 29.31 & 28.34 & - \\
                      & \multicolumn{1}{l|}{BM25 + MonoT5 + date Query}        & - & 26.67 & 26.19 & - \\
                      & \multicolumn{1}{l|}{BM25 + ListT5 + ours} & \textbf{29.11} & \textbf{30.27} & \textbf{29.32} & \textbf{29.57} \\
\noalign{\hrule height 1pt}
\end{tabular}
}
\end{table*}


==> tables/ndcg100.tex <==
\begin{table*}[t]
\centering
\caption{Comparative evaluation of \textbf{nDCG@100} scores between baselines and ours on two year competition datasets. The best performance on each dataset for each method is highlighted in bold.}
\label{tab:ndcg100}
\scalebox{1.0}{
\def\arraystretch{1.0}
\begin{tabular}{c|c|ccc|c}
\noalign{\hrule height 1pt}
\multicolumn{1}{c|}{\textbf{Year}} & \textbf{Method}  & \textbf{Train} & \textbf{Test-Long} & \textbf{Test-Short} & \textbf{Average} \\ 
\hline
\multirow{6}{*}{2023} & 
\multicolumn{1}{l|}{BM25 (uncleaned)}      & 24.23 & 25.27 & 24.72 & 24.74 \\
& \multicolumn{1}{l|}{BM25}                 & 24.20 & 25.46 & 25.02 & 24.89 \\
                      & \multicolumn{1}{l|}{BM25 + MonoT5}        & 28.21 & 29.6 & 28.7 & 28.84 \\
                      & \multicolumn{1}{l|}{BM25 + MonoT5 + 
                      date Document}        & - & 29.31 & 28.34 & - \\
                      & \multicolumn{1}{l|}{BM25 + MonoT5 + date Query}        & - & 26.67 & 26.19 & - \\
                      & \multicolumn{1}{l|}{BM25 + ListT5 + ours} & \textbf{29.11} & \textbf{30.27} & \textbf{29.32} & \textbf{29.57} \\
\noalign{\hrule height 1pt}
% \multirow{6}{*}{2024} & \multicolumn{1}{l|}{BM25 - uncleaned}                 & 29.69 & - & - & - \\
% & \multicolumn{1}{l|}{BM25}                 & 30.34 & - & - & - \\
%                       & \multicolumn{1}{l|}{BM25 + MonoT5}        & 33.32& - & - & - \\
%                       & \multicolumn{1}{l|}{BM25 + MonoT5 + 
%                       date Document}        & Train & - & - & - \\
%                       & \multicolumn{1}{l|}{BM25 + MonoT5 + date Query}        & Train & - & - & - \\
%                       & \multicolumn{1}{l|}{BM25 + ListT5 + ours} & Train & - & - & - \\
% \noalign{\hrule height 1pt}
\end{tabular}
}
\end{table*}


==> utils/configs.tex <==
\useunder{\uline}{\ul}{}
\setsansfont{Calibri}
\setmonofont{Consolas}


